HERD: Continuous Human-to-Robot Evolution for Learning from Human Demonstration

The ability to learn from human demonstration endows robots with the ability to automate various tasks. However, directly learning from human demonstration is challenging since the structure of the human hand can be very different from the desired robot gripper. In this work, we show that manipulation skills can be transferred from a human to a robot through the use of micro-evolutionary reinforcement learning, where a five-finger human dexterous hand robot gradually evolves into a commercial robot, while repeated interacting in a physics simulator to continuously update the policy that is first learned from human demonstration. To deal with the high dimensions of robot parameters, we propose an algorithm for multi-dimensional evolution path searching that allows joint optimization of both the robot evolution path and the policy. Through experiments on human object manipulation datasets, we show that our framework can efficiently transfer the expert human agent policy trained from human demonstrations in diverse modalities to target commercial robots.

==> figure_hand_interp.tex <==

\begin{figure}[t]
\newcommand\sampleheight{0.23}
\centering
\small
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_ff/image_0.00.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_mf/image_0.00.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_ff/image_0.00.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_mf/image_0.00.jpg}
}
\\
\vspace{-2ex}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_ff/image_0.20.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_mf/image_0.20.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_ff/image_0.20.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_mf/image_0.20.jpg}
}
\\
\vspace{-2ex}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_ff/image_0.40.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_mf/image_0.40.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_ff/image_0.40.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_mf/image_0.40.jpg}
}
\\
\vspace{-2ex}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_ff/image_0.60.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_mf/image_0.60.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_ff/image_0.60.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_mf/image_0.60.jpg}
}
\\
\vspace{-2ex}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_ff/image_0.80.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_mf/image_0.80.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_ff/image_0.80.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_mf/image_0.80.jpg}
}
\\
\vspace{-2ex}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_ff/image_1.00.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/cut_mf/image_1.00.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_ff/image_1.00.jpg}
}
\subfloat{
    \includegraphics[height=\sampleheight\linewidth, valign=t]{Figures/hand_interp/merge_mf/image_1.00.jpg}
}
\\
\vspace{-1ex}
\caption{
\textbf{Visualization of Continuous hand evolution towards Rethink gripper.}
From left to right in each row: Cutting evolution \& keep first finger; Cutting evolution \& keep middle finger; Merging evolution \& keep first finger; Merging evolution \& keep middle finger.
From top to bottom, the interpolation from are $[0, 0.2, 0.4, 0.6, 0.8, 1]$ respectively in the six rows.
}
\vspace{-1ex}
\label{fig:hand:interp}
\end{figure}

==> table_dapg.tex <==
\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{1.8pt}
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
& \multirow{2}{*}{Reward} & Demo & \multicolumn{2}{c|}{\texttt{Door}}  & \multicolumn{2}{c|}{\texttt{Hammer}} & \multicolumn{2}{c}{\texttt{Relocate}} \\ \cline{4-9}
& & Agent & \# of sim epochs & \# of train iters & \# of sim epochs & \# of train iters & \# of sim epochs & \# of train iters \\
\hline
\multirow{2}{*}{From Scratch} & Shaped & None & 608700 $\pm$ 79410 & 50725 $\pm$ 6617 & 248460 $\pm$ 9732 & 20705 $\pm$ 811 &   693540 $\pm$ 118860 & 57795 $\pm$ 9905 \\ 
\cline{2-9}
& Sparse & None & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ & $\infty$ \\ 
\hline
DAPG \cite{dapg} & Sparse & Sawyer & 245659 $\pm$ 24934 & 20471 $\pm$ 2077 & 161047 $\pm$ 14027 & 13420 $\pm$ 1168 &  \textbf{114335 $\pm$ 15343} & 9527 $\pm$ 1278 \\
\hline
REvolveR \cite{revolver} & Sparse & ADROIT & 273663 $\pm$ 28236 &	14302 $\pm$ 1843 & 110198 $\pm$ 4407 & 6356 $\pm$ 274 & 163611 $\pm$ 2859 & 8808 $\pm$ 450 \\
\hline
\textbf{HERD (Ours)} & Sparse & ADROIT & \textbf{201190 $\pm$ 23466} & \textbf{11229 $\pm$ 1166}  & \textbf{91674 $\pm$ 6557} & \textbf{4434 $\pm$ 605} & 145158 $\pm$ 4207 & \textbf{8294 $\pm$ 1265} \\ \hline
\end{tabular}
}
\vspace{1ex}
\caption{\textbf{Target Sawyer Robot Performance on Hand Manipulation Suite tasks \cite{dapg}}.
The evaluation metrics is the number of simulation epochs and policy optimization iterations needed to reach 80\% task success rate, shown as the ``mean $\pm$ standard deviation'' from runs with 5 random seeds.
}
\label{tab:dapg:result}
\end{table}

==> table_dapg_v2.tex <==
\begin{table}[t]
\centering
\small
\resizebox{1.0\textwidth}{!}{
\begin{tabular}{l|l|l|l|c|c|c}
\hline
& Reward                  & Demo Agent              &                                          & Door           & Hammer        & Relocate        \\ \hline
\multirow{4}{*}{From Scratch} & \multirow{2}{*}{Shaped} & \multirow{2}{*}{None}   & \# of sim epochs                         & 608700 ± 79410 & 248460 ± 9732 & 693540 ± 118860 \\ \cline{4-7} 
&                         &                         & \# of train iters                        &                &               &                 \\ \cline{2-7} 
& \multirow{2}{*}{Sparse} & \multirow{2}{*}{None}   & \# of sim epochs                         &                &               &                 \\ \cline{4-7} 
&                         &                         & \# of train iters                        &                &               &                 \\ \hline
\multirow{2}{*}{DAPG}         & \multirow{2}{*}{Sparse} & \multirow{2}{*}{Sawyer} & \# of sim epochs                         &                &               &                 \\ \cline{4-7} 
&                         &                         & \# of train iters                        &                &               &                 \\ \hline
\multirow{2}{*}{REvolveR}     & \multirow{2}{*}{Sparse} & \multirow{2}{*}{ADROIT} & \# of sim epochs                         &                &               &                 \\ \cline{4-7} 
&                         &                         & \# of train iters                        &                &               &                 \\ \hline
\multirow{4}{*}{HERD (ours)}  & \multirow{4}{*}{Sparse} & \multirow{4}{*}{ADROIT} & \# of sim epochs for &                &               &                 \\ \cline{4-7} 
&                         &                         & \# of sim epochs for &                &               &                 \\ \cline{4-7} 
&                         &                         & \# of sim epochs                         &                &               &                 \\ \cline{4-7} 
&                         &                         & \# of train iters                        &                &               &                 \\ \hline
\end{tabular}
}
\vspace{1ex}
\caption{\textbf{Target Sawyer Robot Performance on Hand Manipulation Suite tasks \cite{dapg}}.
The evaluation metrics is the number of simulation epochs and policy optimization iterations needed to reach 80\% task success rate, shown as the ``mean $\pm$ standard deviation'' from runs with 5 random seeds.
}
\label{tab:dapg:result}
\vspace{-5ex}
\end{table}

==> table_evo_compare.tex <==
\begin{table*}[h]
\small
\centering
\begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c}
\hline
Task from HMS \cite{dapg} & \multicolumn{4}{c|}{\texttt{door}} & \multicolumn{4}{c|}{\texttt{hammer}} & \multicolumn{4}{c}{\texttt{relocate}} \\ 
\hline
Remaining Finger & \multicolumn{2}{c|}{First Finger} & \multicolumn{2}{c|}{Middle Finger} & \multicolumn{2}{c|}{First Finger} & \multicolumn{2}{c|}{Middle Finger} & \multicolumn{2}{c|}{First Finger} & \multicolumn{2}{c}{Middle Finger} \\ 
\hline
Finger Evolution & Merge & Cut & Merge & Cut & Merge & Cut & Merge & Cut & Merge & Cut & Merge & Cut \\
\hline
\texttt{arm$\rightarrow$hand} & 8.2K & 4.4K & 40.3K & 18.5K & 10.2K & 9.7K & 10.1 & 10.4K & 26.7K & 25.9K & 27.3K & 15.1K \\
\texttt{hand$\rightarrow$arm} & 18.2K & 10.7K & 27.1K & 21.7K & 9.5K & 10.9K & 
8.5K & 11.7K & 51.9K & 24.0K & 42.6K & 29.0K
 \\
\texttt{linear} & 27.3K & 9.1K & 35.0K & 8.4K & 6.4K & 7.5K & 8.6K & 6.8K & 34.0K & 48.6K & 57.9K & 39.5K \\
\hline
\end{tabular} 
\vspace{1ex}
\caption{\textbf{Comparison of different evolution strategies of human hand and arm on different tasks}. Evaluation Metrics are the number of RL iterations for reaching 90\% success rate on the task. 
We show the results of 
}
\label{tab:evolution:strategy:ablation}
\end{table*}
